Learning-Based On-Track System Identification for Scaled Autonomous Racing in Under a Minute

Accurate tire modeling is crucial for optimizing autonomous racing vehicles, as state-of-the-art (SotA) model-based techniques rely on precise knowledge of the vehicle's parameters. Yet, system identification in dynamic racing conditions is challenging due to varying track and tire conditions. Traditional methods require extensive operational ranges, often impractical in racing scenarios. Machine learning (ML)-based methods, while improving performance, struggle with generalization and depend on accurate initialization. This paper introduces a novel on-track system identification algorithm, incorporating a neural network (NN) for error correction, which is then employed for traditional system identification with virtually generated data. Crucially, the process is iteratively reapplied, with tire parameters updated at each cycle, leading to notable improvements in accuracy in tests on a scaled vehicle. Experiments show that it is possible to learn a tire model without prior knowledge with only 30 seconds of driving data and 3 seconds of training time. This method demonstrates greater one-step prediction accuracy than the baseline nonlinear least squares (NLS) method under noisy conditions, achieving a 3.3x lower root mean square error (RMSE), and yields tire models with comparable accuracy to traditional steady-state system identification. Furthermore, unlike steady-state methods requiring large spaces and specific experimental setups, the proposed approach identifies tire parameters directly on a race track in dynamic racing environments.

==> abstract_attempts.tex <==

first attempt, eeeh
Autonomous racing vehicles rely on accurate models for better control and performance. 
\todo{extend motivation}
This paper presents a novel approach to on-track system identification for autonomous racing vehicles, focusing on F1:10 vehicles. Our method integrates a simple \gls{nn} with a nominal Pacejka tire model to enhance the accuracy of lateral dynamics.
The \gls{nn} learns model errors, enabling real-time adaptation to changing conditions and rapid model identification within just a few laps of driving. This makes our approach suitable for dynamic environments.
Furthermore, we extract parameters of the Pacejka model from the \gls{nn}, reducing the need for extensive data collection. This minimal data requirement makes our method practical for real-world applications, where data collection can be challenging. Additionally, the ability to rapidly adjust model parameters enables adaptation to dynamic environments, such as changes in road conditions (e.g., wet roads), ensuring robust performance in various scenarios.
Experimental results demonstrate the effectiveness of our approach, showing significant improvements in lap times and lateral error reduction compared to nominal models.
\todo{add quantifiable metrics}






second attempt, not bad but too long as always..
Accurate tire modeling is crucial for optimizing the performance of autonomous racing vehicles. However, system identification in dynamic racing conditions presents significant challenges, particularly due to varying track and tire conditions. Traditional steady-state identification methods require large operational spaces, which may not be feasible, necessitating the use of on-track methods. Optimization-based methods like \gls{nls} are highly sensitive to outliers, which compromises their robustness. State-of-the-art learning-based approaches compensate for model errors and show improved behavior, however, they often struggle with generalization and typically necessitate initially accurate models, limiting their practical application. In response, this paper introduces a novel learning-based on-track system identification algorithm that integrates a simple \gls{nn} with a nominal Pacejka tire model, effectively capturing real-time tire dynamics for F1TENTH autonomous vehicles, without prior knowledge of the parameters. Our approach begins with modeling residual errors and forming a corrected model. This is followed by steady-state system identification using virtual data generated from the corrected model. The identified parameters are then used as a new nominal model for further learning of residual errors, with the process repeating iteratively until convergence. Our method efficiently utilizes just 30 seconds of driving data and requires only 10 seconds of training time to complete six iterations. It allows for model updates within 2 seconds during each iteration, providing dynamic adaptation to changing conditions. Demonstrated to be eight times more robust than the \gls{nls} method, our approach also yields models comparable to those achieved with traditional steady-state system identification. By leveraging on-track data, it effectively replaces steady-state methods, greatly simplifying the system identification process in dynamic racing environments.

